Envisioning Possibilities and Challenges of AI for Personalized Cancer Care

The use of Artificial Intelligence (AI) in healthcare, including in caring for cancer survivors, has gained significant interest. However, gaps remain in our understanding of how such AI systems can provide care, especially for ethnic and racial minority groups who continue to face care disparities. Through interviews with six cancer survivors, we identify critical gaps in current healthcare systems such as a lack of personalized care and insufficient cultural and linguistic accommodation. AI, when applied to care, was seen as a way to address these issues by enabling real-time, culturally aligned, and linguistically appropriate interactions. We also uncovered concerns about the implications of AI-driven personalization, such as data privacy, loss of human touch in caregiving, and the risk of echo chambers that limit exposure to diverse information. We conclude by discussing the trade-offs between AI-enhanced personalization and the need for structural changes in healthcare that go beyond technological solutions, leading us to argue that we should begin by asking, ``Why personalization?''

==> Paper_Content/6_conclusion.tex <==
%\section{Conclusion}

% Effectively, writing a paper involves: telling the reader what you are going to tell them (introduction), telling them that thing (methodology and findings), and finally telling them what you just told them (conclusion). 

% I find this section to be weird. It is rarely longer than 2 paragraphs. I have sometimes just summarized the whole paper and ended with an open-ended question, other times I have tried to push forward more speculative things. In any case, you have to conclude and there are different ways to go about it.

% One way --- the most common way --- is to simply summarize what you did and learned, and what are the implications of the work. To add cherry on the top, you can end with a provocative question or thought.

% Another way involves stating briefly what you have done and learned. Then using the implications to design, state what direction you are pushing the field. This clearly establishes your overall objective and helps the reader to see which direction you are pushing the field. This is stronger IMHO but it is difficult to write. Usually, you will be tired by the time you reach here so don't make this a high aspiration section just yet.

\section{Conclusion}

This research underscores the urgent need for innovative solutions to the mental health challenges faced by minority cancer survivors. AI holds promise as a tool for creating more equitable, effective, and personalized mental health support systems. However, realizing this potential requires a commitment to ongoing research, ethical technology development, and a deep understanding of the diverse needs of cancer survivors. Future studies should continue to explore and refine AI applications in this space, ensuring that they enhance rather than replace the human elements of care and support.



Our findings suggest that AI should not replace but rather enhance existing healthcare infrastructures. Integrating AI with traditional health services can provide a more robust support system that leverages both technology and human expertise \citet{alowais2023revolutionizing}. This integration should include robust privacy protections and mechanisms to encourage diverse information exposure \citet{chen2024generative}. AI tools should be part of a broader strategy that includes real-time data protection measures and algorithms designed to introduce patients to a variety of information and treatment options, avoiding potential biases and promoting an inclusive approach to care \citet{shah2018next}. By embedding AI tools within established healthcare frameworks, we can enhance the overall quality of care, ensuring that patients receive comprehensive support from both AI and human providers.


By promoting health literacy, AI tools ensure that patients are not mere recipients of care but active partners in their health management.



Algorithms must be transparent and free from biases that could lead to discrimination \citet{}. Ensuring that AI applications protect patient confidentiality and data security is crucial to maintaining trust and integrity in healthcare interactions \citet{}.




creation of echo chambers where only conforming opinions and options are reinforced. These concerns underscored the critical need for AI systems to be developed with robust privacy protections and mechanisms to expose patients to a broad spectrum of information, thereby supporting informed and balanced decision-making.

As we engaged more deeply with these concerns, it became evident that integrating AI tools into existing healthcare structures could not be merely about technological implementation. It must also be about enhancing the agency of cancer survivors, enabling them to actively participate in shaping the care they receive. This involves a continuous dialogue between patients, healthcare providers, and technology designers to ensure that AI tools are used ethically and effectively, supporting not just individual health management but also broader health literacy and empowerment.

This approach broke through the initial reservations of participants about the impersonal nature of technology. By focusing on personal stories and specific needs, we shifted the discussion from abstract AI capabilities to tangible benefits, such as improved access to personalized information and support networks. This shift helped illuminate the potential for AI to play a constructive role in their healthcare journeys, fostering a sense of agency among participants and encouraging them to envision engaging actively with AI as part of their support system.

While the potential of AI in enhancing cancer care is immense, realizing this potential requires a careful, nuanced approach that respects and enhances patient agency and participation. This journey of integration calls for a collaborative effort to ensure that AI tools are not only technologically advanced but also deeply human-centric, promoting a healthcare paradigm that is as democratic and inclusive as it is innovative and efficient.

%%%%%%%%%%%% Revision %%%%%%%%%%%%
This research illuminates the delicate balance required when integrating Artificial Intelligence (AI) into the care of minority cancer survivors. While AI presents a frontier of opportunity for equitable, personalized mental health support, it also raises profound questions about the future of human-centric healthcare. As we consider the capabilities of AI to address disparities and enhance care, we must also grapple with its potential to depersonalize and segregate care processes through automated systems.

By integrating AI, we risk simplifying the complex, diverse needs of cancer survivors into algorithms that may not fully comprehend or adapt to the human experience. The real challenge, then, is not just to advance AI technology but to ensure that it supports a healthcare system where technology complements human expertise, where machines are taught to respect cultural nuances, and where privacy does not become a privilege but remains a right.

Moreover, the development of AI solutions must go hand in hand with efforts to foster health literacy, empowering patients to become informed participants in their care, not passive recipients. This commitment to patient empowerment and informed consent should guide our integration of AI into healthcare, ensuring that these tools enhance rather than undermine the agency of those they are designed to help.

In reimagining AI's role in healthcare, we must also challenge ourselves to think beyond the immediate benefits of technology. How do we design AI systems that reinforce the human elements of empathy, understanding, and care? How do we prevent AI from isolating patients within echo chambers of their own health data? These questions compel us to consider AI not just as a technological tool but as a participant in the broader discourse on ethical, patient-centered care.

Engaging with these complex issues requires a multidimensional approach that encompasses not only technological development but also regulatory frameworks, patient education, and a recommitment to the core values of healthcare. As we move forward, our focus should remain steadfast on enhancing the symbiosis between AI and human care providers, ensuring that together they create a more responsive, inclusive, and compassionate healthcare system.

==> Paper_Content/discussion_ideas.tex <==
We note that in envisioning AI for healthcare, particularly for mental health, there is a risk for people to be pacified and not demand changes of the existing structures. 



==> Paper_Content/old_methodology.tex <==
\section{Data Collection and Analysis}

%\subsection{Participant Description}
 %This diversity is crucial for understanding the broad spectrum of informational needs and behaviors among cancer survivors. %Participants' demographic information is listed in Table 1.


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\caption{Participant demographics. All the data are self-reported.}
\vspace{-1em}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllll}
\hline
\multicolumn{1}{c}{\textbf{ID}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Age \\ Range\end{tabular}}} & \multicolumn{1}{c}{\textbf{Gender}} & \multicolumn{1}{c}{\textbf{Race/ Ethnicity}} & \multicolumn{1}{c}{\textbf{Cancer Type}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Stage at \\ Diagnosis\end{tabular}}} & \multicolumn{1}{c}{\textbf{Current Stage}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Treatment(s) \\ so far\end{tabular}}} \\ \hline
P1 & 45-54 & Female & \begin{tabular}[c]{@{}l@{}}Black or African \\ American\end{tabular} & Breast & Stage II & In remission & \begin{tabular}[c]{@{}l@{}}Chemotherapy, \\ Surgery\end{tabular} \\ \hline
P2 & 45-54 & \begin{tabular}[c]{@{}l@{}}Prefer not \\ to say\end{tabular} & \begin{tabular}[c]{@{}l@{}}I describe myself \\ in some other way\end{tabular} & Melanoma & Stage II & Stage I & Radiation therapy \\ \hline
P3 & 25-34 & Male & Asian & Prostate & Stage II & In remission & Surgery \\ \hline
P4 & 55-64 & Female & Asian & Lung & Stage II & In remission & \begin{tabular}[c]{@{}l@{}}Chemotherapy, Radiation \\ therapy, Surgery\end{tabular} \\ \hline
P5 & 45-54 & Male & Asian & Lung & Stage I & In remission & Surgery \\ \hline
P6 & 65+ & Female & Asian & Colorectal & Stage I & In remission & Chemotherapy, Surgery \\ \hline
\end{tabular}%
}
\vspace{-0.5em}
\end{table*}






% The quantitative component, consisting of responses from six questionnaires, was subjected to statistical analysis. The aim was to quantitatively assess patterns and trends in health information-seeking behaviors among cancer patients and their perceptions of AI in mental health care.

% Most participants identified as female (n = 3, 50\%), with the others being male (n = 2, 33.3\%) and one preferring not to specify their gender (n = 1, 16.7\%). At the time the study concluded, participant ages varied from 25 to over 65. Half of the participants (n = 3) were aged between 45 and 54, while one participant 16.7\% (n = 1) of 25-34, 55-64 and 65+ respectively. In terms of ethnicity, 66.7\% of the participants (n = 4) were Asian, 16.7\% (n = 1) were Black or African American, and one participant chose to describe their ethnicity in another way. Participants reported a variety of cancer diagnoses, stages of remission, and treatment approaches. Six participants disclosed their type of cancer; lung cancer was among the most frequently reported diagnoses (n = 2, 33.3\%), breast (n = 1, 16.7\%), prostate (n = 1, 16.7\%), colorectal (n = 1, 16.7\%), and melanoma (n = 1, 16.7\%). The majority of the study participants were diagnosed with Stage II cancer (n = 4, 66.7\%), while the remaining two participants (33.3\%) were diagnosed with Stage I cancer (33.3%). In the current staging, most participants (n = 5, 83.3\%) were in full remission, with one participant (16.7%) at Stage I. Treatment types varied; 83.3\% (n = 5) underwent surgical treatment, 50% (n = 3) underwent chemotherapy, and 2 participants reported receiving radiation therapy (33.3%). It is noteworthy that several participants underwent multiple forms of treatment.



%\subsection{Data Collection and Analysis}

As part of our pilot study, we interviewed six cancer survivors from diverse backgrounds, ensuring a representation of varied cancer types and stages (see Table \ref{tab:my-table}). 
The interviews were between 45 to 90 minutes long. All of the interviews were remotely conducted considering the participants' preferences and geographical constraints. 
We recorded the audio.

We conducted thematic analysis of the transcript, starting from open-coding and iteratively working towards higher-level codes. Following Salda{\~n}a's guidelines for ``solo coding'' \cite{saldana2021coding}, the first author, who did the open coding alone, consulted and discussed the emerging codes with the last author throughout the coding process.  Intermediate categories that emerged included ``Experience with Current Interventions,'' ``Unique Needs and Challenges,'' and ``Perception and Openness to AI-based Solutions.'' 
Subsequently, we ended with the high-level codes such as ``Desired Outcomes and Features,'' ``Integration and Accessibility,'' and ``Trust and Reliability.''


==> Paper_Content/questionnaire_table.tex <==
\section{Appendix}

\begin{table}[hf]
\caption{Summary statistics of the participants' response to our questionnaire about AI's role}
\begin{tabular}{lll}
\hline
\multicolumn{1}{|l|}{\textbf{Items}} & \multicolumn{1}{l|}{\textbf{Mean}} & \multicolumn{1}{l|}{\textbf{SD}} \\ \hline
\textbf{Experience with Current Interventions} &  &  \\ \hline
\multicolumn{1}{|l|}{I am   satisfied with the mental health support available to me as a cancer   survivor.} & \multicolumn{1}{l|}{15.67} & \multicolumn{1}{l|}{1.506} \\ \hline
\multicolumn{1}{|l|}{The   mental health services I have accessed were effective in addressing my needs.} & \multicolumn{1}{l|}{16} & \multicolumn{1}{l|}{1.265} \\ \hline
\multicolumn{1}{|l|}{I have   faced barriers in accessing mental health services (e.g., financial,   geographical, stigma).} & \multicolumn{1}{l|}{17.83} & \multicolumn{1}{l|}{0.983} \\ \hline
\multicolumn{1}{|l|}{The   mental health support I received was tailored to my experiences as a cancer   survivor.} & \multicolumn{1}{l|}{14.67} & \multicolumn{1}{l|}{1.033} \\ \hline
\textbf{Unique   Needs and Challenges} &  &  \\ \hline
\multicolumn{1}{|l|}{I feel   that my mental health challenges are unique compared to those who have not   experienced cancer.} & \multicolumn{1}{l|}{14.67} & \multicolumn{1}{l|}{0.516} \\ \hline
\multicolumn{1}{|l|}{Current   mental health services adequately address the fear of cancer recurrence.} & \multicolumn{1}{l|}{11} & \multicolumn{1}{l|}{2} \\ \hline
\multicolumn{1}{|l|}{I need   more support in managing the long-term emotional impact of cancer than is   currently available.} & \multicolumn{1}{l|}{14.33} & \multicolumn{1}{l|}{0.516} \\ \hline
\textbf{Perception   and Openness to AI-based Solutions} &  &  \\ \hline
\multicolumn{1}{|l|}{I am open to using AI-based tools for mental health support.} & \multicolumn{1}{l|}{13.17} & \multicolumn{1}{l|}{1.329} \\ \hline
\multicolumn{1}{|l|}{I   believe AI can offer personalized mental health support tailored to my needs   as a cancer survivor.} & \multicolumn{1}{l|}{13.33} & \multicolumn{1}{l|}{1.033} \\ \hline
\multicolumn{1}{|l|}{Privacy   concerns would deter me from using AI-based mental health solutions.} & \multicolumn{1}{l|}{14.17} & \multicolumn{1}{l|}{0.408} \\ \hline
\textbf{Desired Outcomes and Features} &  &  \\ \hline
\multicolumn{1}{|l|}{I would prefer an AI-based mental health solution that understands and responds to my   emotions effectively.} & \multicolumn{1}{l|}{13.5} & \multicolumn{1}{l|}{1.225} \\ \hline
\multicolumn{1}{|l|}{Continuous   access to AI-based mental health support would be beneficial for managing my   condition.} & \multicolumn{1}{l|}{13.33} & \multicolumn{1}{l|}{1.033} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}It is   important for AI-based solutions to offer strategies for coping with stress   and anxiety specific to cancer \\ survivorship.\end{tabular}} & \multicolumn{1}{l|}{13.5} & \multicolumn{1}{l|}{1.225} \\ \hline
\textbf{Integration   and Accessibility} & \textbf{} & \textbf{} \\ \hline
\multicolumn{1}{|l|}{I would   use an AI-based mental health tool more if it were integrated with my   existing healthcare services.} & \multicolumn{1}{l|}{13.67} & \multicolumn{1}{l|}{0.816} \\ \hline
\multicolumn{1}{|l|}{AI-based   mental health solutions should be accessible across various devices and   platforms for convenience.} & \multicolumn{1}{l|}{14.33} & \multicolumn{1}{l|}{0.516} \\ \hline
\textbf{Trust and Reliability} &  &  \\ \hline
\multicolumn{1}{|l|}{I would   trust an AI-based system to keep my mental health information confidential.} & \multicolumn{1}{l|}{11.67} & \multicolumn{1}{l|}{1.506} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}It is   crucial that AI-based mental health solutions are developed with input from   healthcare professionals and\\ cancer survivors.\end{tabular}} & \multicolumn{1}{l|}{14.67} & \multicolumn{1}{l|}{0.516} \\ \hline
\end{tabular}
\label{tab:questionnaire}
\end{table}



% \begin{table}[]
% \begin{tabular}{@{}lll@{}}
% \toprule
% \textbf{Items} & \textbf{Mean} & \textbf{SD} \\ \midrule
% \textbf{Experience with Current Interventions} &  &  \\ \midrule
% \multicolumn{1}{|l|}{I am   satisfied with the mental health support available to me as a cancer   survivor.} & \multicolumn{1}{l|}{15.67} & \multicolumn{1}{l|}{1.506} \\ \midrule
% \multicolumn{1}{|l|}{The   mental health services I have accessed were effective in addressing my needs.} & \multicolumn{1}{l|}{16} & \multicolumn{1}{l|}{1.265} \\ \midrule
% \multicolumn{1}{|l|}{I have   faced barriers in accessing mental health services (e.g., financial,   geographical, stigma).} & \multicolumn{1}{l|}{17.83} & \multicolumn{1}{l|}{0.983} \\ \midrule
% \multicolumn{1}{|l|}{The   mental health support I received was tailored to my experiences as a cancer   survivor.} & \multicolumn{1}{l|}{14.67} & \multicolumn{1}{l|}{1.033} \\ \midrule
% \textbf{Unique   Needs and Challenges} &  &  \\ \midrule
% \multicolumn{1}{|l|}{I feel   that my mental health challenges are unique compared to those who have not   experienced cancer.} & \multicolumn{1}{l|}{14.67} & \multicolumn{1}{l|}{0.516} \\ \midrule
% \multicolumn{1}{|l|}{Current   mental health services adequately address the fear of cancer recurrence.} & \multicolumn{1}{l|}{11} & \multicolumn{1}{l|}{2} \\ \midrule
% \multicolumn{1}{|l|}{I need   more support in managing the long-term emotional impact of cancer than is   currently available.} & \multicolumn{1}{l|}{14.33} & \multicolumn{1}{l|}{0.516} \\ \midrule
% \textbf{Perception   and Openness to AI-based Solutions} &  &  \\ \midrule
% \multicolumn{1}{|l|}{I am open to using AI-based tools for mental health support.} & \multicolumn{1}{l|}{13.17} & \multicolumn{1}{l|}{1.329} \\ \midrule
% \multicolumn{1}{|l|}{I   believe AI can offer personalized mental health support tailored to my needs   as a cancer survivor.} & \multicolumn{1}{l|}{13.33} & \multicolumn{1}{l|}{1.033} \\ \midrule
% \multicolumn{1}{|l|}{Privacy   concerns would deter me from using AI-based mental health solutions.} & \multicolumn{1}{l|}{14.17} & \multicolumn{1}{l|}{0.408} \\ \midrule
% \textbf{Desired Outcomes and Features} &  &  \\ \midrule
% \multicolumn{1}{|l|}{I would prefer an AI-based mental health solution that understands and responds to my   emotions effectively.} & \multicolumn{1}{l|}{13.5} & \multicolumn{1}{l|}{1.225} \\ \midrule
% \multicolumn{1}{|l|}{Continuous   access to AI-based mental health support would be beneficial for managing my   condition.} & \multicolumn{1}{l|}{13.33} & \multicolumn{1}{l|}{1.033} \\ \midrule
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}It is   important for AI-based solutions to offer strategies for coping with stress   and anxiety specific to cancer \\ survivorship.\end{tabular}} & \multicolumn{1}{l|}{13.5} & \multicolumn{1}{l|}{1.225} \\ \midrule
% \textbf{Integration   and Accessibility} & \textbf{} & \textbf{} \\ \midrule
% \multicolumn{1}{|l|}{I would   use an AI-based mental health tool more if it were integrated with my   existing healthcare services.} & \multicolumn{1}{l|}{13.67} & \multicolumn{1}{l|}{0.816} \\ \midrule
% \multicolumn{1}{|l|}{AI-based   mental health solutions should be accessible across various devices and   platforms for convenience.} & \multicolumn{1}{l|}{14.33} & \multicolumn{1}{l|}{0.516} \\ \midrule
% \textbf{Trust and Reliability} &  &  \\ \midrule
% \multicolumn{1}{|l|}{I would   trust an AI-based system to keep my mental health information confidential.} & \multicolumn{1}{l|}{11.67} & \multicolumn{1}{l|}{1.506} \\ \midrule
% \begin{tabular}[c]{@{}l@{}}It is   crucial that AI-based mental health solutions are developed with input from   healthcare professionals and\\ cancer survivors.\end{tabular} & 14.67 & 0.516 \\ \bottomrule
% \end{tabular}
% \end{table}
